Toward Accurate and Realistic Outfits Visualization with Attention to Details

Virtual try-on methods aim to generate images of fashion models wearing arbitrary combinations of garments. This is a challenging task because the generated image must appear realistic and accurately display the interaction between garments. Prior works produce images that are filled with artifacts and fail to capture important visual details necessary for commercial applications. We propose Outfit Visualization Net (OVNet) to capture these important details (e.g. buttons, shading, textures, realistic hemlines, and interactions between garments) and produce high quality multiple-garment virtual try-on images. OVNet consists of 1) a semantic layout generator and 2) an image generation pipeline using multiple coordinated warps. We train the warper to output multiple warps using a cascade loss, which refines each successive warp to focus on poorly generated regions of a previous warp and yields consistent improvements in detail. In addition, we introduce a method for matching outfits with the most suitable model and produce significant improvements for both our and other previous try-on methods. Through quantitative and qualitative analysis, we demonstrate our method generates substantially higher-quality studio images compared to prior works for multi-garment outfits. An interactive interface powered by this method has been deployed on fashion e-commerce websites and received overwhelmingly positive feedback.

==> fashion arxiv paper/figures/OVNet-framework.tex <==
\begin{figure*}
\begin{center}
   \includegraphics[width=0.8\linewidth]{images/OVNet-framework.jpg}
\end{center}
           \vspace{-0.35cm}  

   \caption{{\bf Outfit Visualization Net}, which synthesizes an image of a model wearing multiple garments, consists of two components. The Semantic Layout Generator $G_{layout}$ (left) takes in the garment image $x$, the pose representation $p$ and an incomplete semantic layout $m_i$, and learns to reconstruct the ground truth layout $m$. The multi-warp garment generator $G_{garment}$ (right) has two modules. The {\bf warping module} is a spatial transformer that takes in the garment image $x$ and its semantic layout $m^c$ and regress $k$ sets of transformation parameters ${\theta_1..\theta_k}$. It then samples $k$ warps $w_1..w_k$ where $ w_1=\mathcal{W}(x,\theta_1)$, using the predicted transformations. The {\bf inpainting module} takes in the predicted warps ${w_1..w_k}$, the full semantic layout $m'$, the skin color channel $s$ (median color of the face) and the incomplete model image $y_i$ and generates the final image $y'$ of the model wearing garment $x$. Two modules are trained jointly.
   }
\vspace{-0.5cm}  

\label{fig:meta_figure}
\end{figure*}


==> fashion arxiv paper/figures/amazon_compare.tex <==
 \begin{figure}
\begin{center}
\vspace{-0.5cm}  
	\includegraphics[width=0.99\linewidth]{images/amazon_compare.jpg}
    \caption{We compare visual results between O-VITON~\cite{Neuberger_2020_CVPR} and ours. The top rows show the garments in the oufit and the bottom row shows the generated try-on results. For fair comparison, we found garment images that most closely resemble the garments chosen in~\cite{Neuberger_2020_CVPR} in terms of style, color, and texture. Image results for O-VITON are directly taken from their paper. There are substantial difference in quality between results. The unnaturally flat torso and uneven shoulders of A-1 are not present in B-1. In A-2, the buttons on the jacket are distorted/missing, whereas B-2 represents them accurately. In A-3, the jacket and top lack realism due to missing creases, folds, and bumps compared to B-3. Properties of the arms are also kept intact in B-3. (See Appendix for more)}    
    \label{fig:amazon_compare}
    \end{center}
\vspace{-0.5cm}  
\end{figure}


==> fashion arxiv paper/figures/bad_examples.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.95\linewidth]{images/bad_examples.pdf}
\end{center}
\vspace{-0.3cm}  

    \caption{Our method has forgiving failure modes. When it fails, it still outputs an image of the person wearing realistic garments, but with misrepresented attributes. In A, it turns spaghetti straps into thick straps, and has difficulty with laces; in B, the coat is generated as open-back; the asymmetrical neckline in C is turned into panels; and transparency is not captured in D.}    
    \label{fig:bad_examples}
           \vspace{-0.5cm}  

\end{figure}

==> fashion arxiv paper/figures/generation_examples.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.99\linewidth]{images/header.png}
\end{center}
           \vspace{-0.5cm}  
    \caption{Our method takes in a model image and multiple neutral garments images as inputs, and generates a high quality image of the selected model wearing the garments. {\bf Pay careful attention to details} of the garment properties that are accurately portrayed (e.g., the patterns on the dress (A-1), the unicorn and the string (C-2), the hemline (C-2), buttons (B-1, D-2), and the lengths of the garments); the interaction between multiple garments has been captured (e.g., the collar and sleeve coming out of the sweater (A-1), the open outerwear cast shading (B-1, C-2) to the garment beneath); the interaction between the garment and the person is natural (e.g., the loose sleeves, the folds by the arm (D-2), and the shadows casted on the leg by the dresses); and skin is generated realistically (B-1). See image without bounding box in Appendix.}  
       \vspace{-0.5cm}  
          \label{fig:header}
\end{figure}

==> fashion arxiv paper/figures/good-bad_matching.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.9\linewidth]{images/good-bad_matching.pdf}
\end{center}
           \vspace{-0.3cm}  
    \caption{This figure shows an example result from a matched garment-pose pair versus a non-matched pair. A model $y$ with extracted pose $p$ is fed two different outfits $O_1$ and $O_2$. The garments in $O_1$ match with the shape of garments worn by the original model $y$, thus results in an accurate layout prediction $m_1'$ and output $y_1'$. In contrast, the sleeveless tank in $O_2$ does not match with pose $p$, thus was wrongly generated with sleeves in $y_2'$.}    
    \label{fig:good-bad_matching}
           \vspace{-0.3cm}  
\end{figure}

==> fashion arxiv paper/figures/layout_generator.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.99\linewidth]{images/layout_generator.pdf}
\end{center}
           \vspace{-0.5cm}  
    \caption{The layout generator takes in the garment image $x$, the pose representation $p$ and an incomplete semantic layout $m_i$, and learns to reconstruct the ground truth layout $m$.
    }    
\label{fig:layout_generator}
\vspace{-0.5cm}  

\end{figure}

==> fashion arxiv paper/figures/model_pose.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.99\linewidth]{images/model-pose.jpg}
\end{center}
           \vspace{-0.3cm}  
    \caption{We notice that the human pose annotation from OpenPose embeds information differently depending on the type of garment. For example, the pose predictor consistently predicts wider distance between shoulder and elbow anchor for models wearing coats (3, 4) than models wearing shirts (1, 2), despite both models having similar posture and body shape. This implies that the pairing between pose and garments can influence the predicted layout.
    }  
    \label{fig:model_pose}
       \vspace{-0.5cm}  

\end{figure}


==> fashion arxiv paper/figures/multi_warp.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=.9\linewidth]{images/multi_warp_generation.png}
\end{center}
   \caption{We use a warping process to place garment on models. Uing multiple coordinated warpers outperforms a single warper, especially when the garment have multiple disconnected components (e.g., an unzipped jacket). Our warpers are trained such that the second warper will address error made by the first warper and so long. Having multiple warps requires the final rendering module to know which warp to rely on for different areas. We use a modified inpainting network that takes in the masked model ($m_i^t \otimes x_i$) and each warpers' output. This network learns to combine warps and inpaint the masked region of the model.
\vspace{-0.5cm}
}
\label{fig:synthesis-net}
\end{figure}

==> fashion arxiv paper/figures/multi_warp_vs_single.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=.95\linewidth]{images/multi-warp-qualitative.jpg}
\end{center}
\vspace{-0.3cm}  
   \caption{ The figures shows qualitative comparison between using multiple (2) warpers and a single warper. Note for single warp: the buttons are in the wrong place in A and D; problems with sleeve boundaries in E; a severe misalignment in C; a misplaced tag in B. All problems are fixed in multi-warp results.
}
   \label{fig:multi-warp-qualitative}
          \vspace{-0.3cm}  

\end{figure}


==> fashion arxiv paper/figures/multiple_models.tex <==
 \begin{figure}
\begin{center}
\vspace{-0.2cm}  
	\includegraphics[width=0.99\linewidth]{images/multiple_models.pdf}
    \caption{We show a sequence of visualizations for the same outfit generated on different reference models. Our generation method is able to adapt to a diverse set of poses, skin-tones, and hand positions. When the hand is in the pocket, the jeans plump up and connect seamlessly with the jacket (Pose 2 \& 5).}    
    \label{fig:multiple_models}
    \end{center}
\vspace{-0.8cm}  
\end{figure}

==> fashion arxiv paper/figures/pose_germent_matching.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=.95\linewidth]{images/pose_garment_matching.pdf}
\end{center}
\vspace{-0.5cm}

   \caption{ This figure shows the training procedure for the garment-pose matching embedding. We obtained a foreground mask $z_a$ from garment image $x_a$, and learn a shape Auto-encoder $\{E_s, D_s\}$ to produce a shape embedding. The pose $p_a$ from the corresponding model $y_a$ is embedded closer to $z_a$ than a random pose $p_b$. This only works for scenarios {\bf (a) and (b)} (from Intro~\ref{sec:intro})
   }
   \vspace{-0.5cm}
\label{fig:pose_germent_matching}
\end{figure}


==> fashion arxiv paper/figures/sequence_change.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=1\linewidth]{images/sequence_change.jpg}
\end{center}
           \vspace{-0.3cm}  
   \caption{ The figure shows a sequence of outfit visualizations produced by our method on two different models. Our method can modify one garment at a time, leaving the rest of the image untouched. The details of the garments' shape are accurately represented (e.g., neckline shape, skirt length, pant width, etc.) and consistent on both models. The garment interactions of the top (hanging or tucked-in) also vary between poses.
}
       \vspace{-0.5cm}  

   \label{fig:outfit-visualization}
\end{figure}


==> fashion arxiv paper/figures/user-study-examples.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=0.95\linewidth]{images/user-study-examples.jpg}
\end{center}
\vspace{-0.3cm}  

   \caption{ Two synthesized images that 70\% of the participants in the user study thought were real. 
Note, e.g., the shading, the wrinkles, even the zip and the collar.
   }
\label{fig:user-study-examples}
\vspace{-0.3cm}  

\end{figure}


==> figures/layout_generator.tex <==
 \begin{figure}
\begin{center}
   \includegraphics[width=0.99\linewidth]{images/layout_generator.pdf}
\end{center}
           \vspace{-0.5cm}  
    \caption{The layout generator takes in the garment image $x$, the pose representation $p$ and an incomplete semantic layout $m_i$, and learns to reconstruct the ground truth layout $m$.
    }    
\label{fig:layout_generator}
\vspace{-0.5cm}  

\end{figure}

==> figures/multi_warp.tex <==
\begin{figure}
\begin{center}
   \includegraphics[width=.9\linewidth]{images/multi_warp_generation.png}
\end{center}
   \caption{We use a warping process to place garment on models. Uing multiple coordinated warpers outperforms a single warper, especially when the garment have multiple disconnected components (e.g., an unzipped jacket). Our warpers are trained such that the second warper will address error made by the first warper and so long. Having multiple warps requires the final rendering module to know which warp to rely on for different areas. We use a modified inpainting network that takes in the masked model ($m_i^t \otimes x_i$) and each warpers' output. This network learns to combine warps and inpaint the masked region of the model.
\vspace{-0.5cm}
}
\label{fig:synthesis-net}
\end{figure}
